Statistical Inference on Explained Variation in High-dimensional Linear Model with Dense Effects

Statistical inference on the explained variation of an outcome by a set of covariates is of particular interest in practice. When the covariates are of moderate to high-dimension and the effects are not sparse, several approaches have been proposed for estimation and inference. One major problem with the existing approaches is that the inference procedures are not robust to the normality assumption on the covariates and the residual errors. In this paper, we propose an estimating equation approach to the estimation and inference on the explained variation in the high-dimensional linear model. Unlike the existing approaches, the proposed approach does not rely on the restrictive normality assumptions for inference. It is shown that the proposed estimator is consistent and asymptotically normally distributed under reasonable conditions. Simulation studies demonstrate better performance of the proposed inference procedure in comparison with the existing approaches. The proposed approach is applied to studying the variation of glycohemoglobin explained by environmental pollutants in a National Health and Nutrition Examination Survey data set.

==> app.tex <==
\begin{center}Appendix I: Proofs of theorems 1 and 2\end{center}

The proofs of the theorems use the Marchenko-Pastur limit law for the empirical covariance matrix of a random matrix,  we list the law here for easy reference. Let $Z_{n\times p}=(Z_{ij})$ where $Z_{ij}, i=1,\cdots, n; j=1,\cdots,p$ are iid with $E(Z_{ij})=0$ and $E(Z_{ij}^{2})=1$. Let
$
M=\frac{1}{p}Z_{n\times p}Z_{n\times p}^{t}.
$
Let the eigenvalues of $M$ be $\eta_{1},\cdots,\eta_{n}$.  Define the empirical spectral measure as
$$
\mu_{n}(A)=\frac{1}{n}\sum_{i=1}^{n}1_{\{\eta_{i}\in A\}}.
$$
Let $n/p\rightarrow \xi$ as $n,p\rightarrow \infty$, where $\xi\in (0,\infty)$. Then $\mu_{n}\rightarrow \mu$ in distribution, where 
$$
\mu(A)=\left\{\begin{array}{ll}
(1-1/\xi) 1_{\{0\in A\}} +\nu(A)          & \mbox{if } \xi >1,  \\
\nu(A)                                                 &\mbox{if } 0<\xi\leq 1,
\end{array}\right.
$$
and the measure $\nu$ has density
$$
d\nu(u)=\frac{1_{\{x\in [a, b]\}}}{2\pi x\xi}\sqrt{(x-a)(b-x)}.
$$
 and $a=(1-\sqrt{\xi})^{2}$ and $b=(1+\sqrt{\xi})^{2}$.

\vspace{0.7cm}

\noindent Proof of Theorem 1: Consider first the case where $n\geq p$. Let the singular value decomposition be
$$
Z_{n\times p}=U_{n\times p}D_{p\times p}V_{p\times p} ^{t},
$$
where $U^{t}U=I_{p\times p}$ and $V^{t}V=VV^{t}=I_{p\times p}$, and $D=\mbox{diag}(d_{1},\cdots,d_{p})$. Let $U^{*}_{n\times(n-p)}$ be the matrix such that
$$
(U,U^{*})^{t}(U,U^{*})=(U,U^{*})(U,U^{*})^{t}=I_{n\times n}.
$$
For $0\leq \lambda<1$, it follows that
$$
I_{n\times n}+\lambda M=(U,U^{*})
\left(\begin{array}{cc}
I_{p\times p}+\lambda D^{2}/p &0 \\
0 & I_{(n-p)\times (n-p)}
\end{array}\right)(U,U^{*})^{t}.
$$
Let $\eta_{k}=d_{k}^{2}/p, k=1,\cdots,p$. We then have
\begin{eqnarray*}
(I_{n\times n}+\lambda M)^{-1}
&=&I_{n\times n}- U\mbox{diag}\left(\frac{\lambda\eta_{1}}{1+\lambda\eta_{1}},\cdots,\frac{\lambda\eta_{p}}{1+\lambda\eta_{p}}\right)U^{t},
\end{eqnarray*}
and
$
W_{\lambda}=U\left(\Delta+I_{p\times p}\right)U^{t}-I_{n\times n},
$
where
$$
\Delta=\mbox{diag}\left(\frac{\eta_{1}-1}{(1+\lambda \eta_{1})^{2}},\cdots,\frac{\eta_{p}-1}{(1+\lambda \eta_{p})^{2}}\right).
$$
It follows that
\begin{eqnarray*}
tr\left\{W_{\lambda}(M-I)\right\}&=&\sum_{k=1}^{p}\frac{(\eta_{k}-1)^{2}}{(1+\lambda \eta_{k})^{2}}+n-p, \\
tr\left\{W_{\lambda}(YY^{t}-I)\right\}&=&Y^{t}(U\Delta U^{t}-U^{*}U^{*t})Y-\sum_{k=1}^{p}\frac{\eta_{k}-1}{(1+\lambda \eta_{k})^{2}}+n-p,
\end{eqnarray*}
Note from $U^{*t}U=0$ that $U^{*t}Z=0$. It follows that
\begin{eqnarray*}
Y^{t}(U\Delta U^{t}-U^{*}U^{*t})Y&=&(Z\alpha)^{t}U\Delta U^{t}Z\alpha+2 (Z\alpha)^{t}U\Delta U^{t}\epsilon +\epsilon^{t}(U\Delta U^{t}-U^{*}U^{*t})\epsilon.
\end{eqnarray*}
It follows from the law of large number for sum of independent variables and for quadratic forms (See the supplemental material for verifying conditions for convergence) that $n^{-1}(Z\alpha)^{t}U\Delta U^{t}\epsilon\rightarrow 0$ in probability and that 
$$
\frac{1}{n}\left[\epsilon^{t}(U\Delta U^{t}-U^{*}U^{*t})\epsilon-E\left\{\epsilon^{t}(U\Delta U^{t}-U^{*}U^{*t})\epsilon\mid Z\right\}\right]\rightarrow 0, 
$$
in probability. These imply that
$$
\frac{1}{n}\left[Y^{t}(U\Delta U^{t}-U^{*}U^{*t})Y-(Z\alpha)^{t}U\Delta U^{t}Z\alpha-E\left\{\epsilon^{t}(U\Delta U^{t}-U^{*}U^{*t})\epsilon\mid Z\right\}\right]\rightarrow 0, 
$$
in probability. Next, $(Z\alpha)^{t}U\Delta U^{t}Z\alpha-tr(Z^{t}U\Delta U^{t}Z/p)r^{2}=0$  when $\alpha=0$. When $\alpha\neq 0$, 
\begin{eqnarray*}
(Z\alpha)^{t}U\Delta U^{t}Z\alpha-tr(Z^{t}U\Delta U^{t}Z/p)r^{2} 
&=&p\left\{\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}v_{k}^{2}(u)-\frac{1}{p}\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}r^{2},
\end{eqnarray*}
where 
$
(v_{1}(u),\cdots,v_{p}(u))^{t}=V^{t}u,
$
$u=\alpha/||\alpha||_{2}$, and $||\alpha||_{2}^{2}=\sum_{j=1}^{p}\alpha_{j}^{2}=r^{2}$. Note that
$$
\frac{x(x-1)}{(1+\lambda x)^{2}}
$$
is a bounded function on $x\geq 0$ for $\lambda>0$. From the convergence results on the eigenvectors of the random covariance matrix (Bai et al, 2007, Corollary 2 of Theorem 1), it follows that
$$
\left\{\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}v_{k}^{2}(u)-\frac{1}{p}\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}\rightarrow 0, a.s.
$$ 
Note here that the convergence also holds when $\lambda=0$ because of the bounded support of the limited spectral distribution. See also Silverstein (1989).  Furthermore,
\begin{eqnarray*}
E\left\{\epsilon^{t}(U\Delta U^{t}-U^{*}U^{*t})\epsilon\mid Z\right\}&=&(1-r^{2})\left\{\sum_{k=1}^{p}\frac{\eta_{k}-1}{(1+\lambda \eta_{k})^{2}}-(n-p)\right\}, \\
tr(Z^{t}U\Delta U^{t}Z/p)r^{2}&=&r^{2}\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda \eta_{k})^{2}},
\end{eqnarray*}
It follows that
\begin{eqnarray*}
\frac{1}{n}\left[Y^{t}(U\Delta U^{t}-U^{*}U^{*t})Y-\sum_{k=1}^{p}\frac{\eta_{k}-1}{(1+\lambda \eta_{k})^{2}}+n-p 
-r^{2}\left\{\sum_{k=1}^{p}\frac{(\eta_{k}-1)^{2}}{(1+\lambda \eta_{k})^{2}}+n-p\right\}\right]&\rightarrow&  0
\end{eqnarray*}
in probability. By the Marchenko-Pastur limit law,
\begin{eqnarray*}
\frac{1}{n}tr\left\{W_{\lambda}(M-I)\right\}&\rightarrow& C=\int_{a}^{b}\frac{(x-1)^{2}}{(1+\lambda x)^{2}}d\nu(x)+(1-1/\xi)1_{\{\xi> 1\}}>0.
\end{eqnarray*}
Since almost sure convergence implies convergence in probability, these put together  imply 
$$
\hat{r}_{\lambda}^{2}\rightarrow r^{2}, 
$$
in probability. It is now straightforward to see that $\hat{\sigma}_{s}^{2}\rightarrow \sigma_{s}^{2}$ and  $\hat{\sigma}_{\epsilon}^{2}\rightarrow \sigma_{\epsilon}^{2}$ in probability.

For $n<p$,  let the singular value decomposition be
$$
Z_{n\times p}=U_{n\times n}D_{n\times n}\{V_{p\times n}\} ^{t},
$$
where $U^{t}U=UU^{t}=I_{n\times n}$ and $V^{t}V=I_{n\times n}$, and $D=\mbox{diag}(d_{1},\cdots,d_{n})$. 
It follows that
\begin{eqnarray*}
W_{\lambda}&=&U\mbox{diag}\left(\frac{\eta_{1}-1}{(1+\lambda\eta_{1})^{2}},\cdots,\frac{\eta_{n}-1}{(1+\lambda \eta_{n})^{2}}\right)U^{t}.
\end{eqnarray*}
We have
\begin{eqnarray*}
\frac{1}{n}tr\left\{W_{\lambda}(M-I)\right\}&=&\frac{1}{n}\sum_{k=1}^{n}\frac{(\eta_{k}-1)^{2}}{(1+\lambda \eta_{k})^{2}}, \\
           &\rightarrow& \int \frac{(x-1)^{2}}{(1+\lambda x)^{2}}dv(x)>0, \\
tr\left\{W_{\lambda}(YY^{t}-I)\right\}&=&Y^{t}U\Delta U^{t}Y-\sum_{k=1}^{n}\frac{\eta_{k}-1}{(1+\lambda \eta_{k})^{2}}.
\end{eqnarray*}
Note further that
$$
Y^{t}U\Delta U^{t}Y=(Z\alpha)^{t}U\Delta U^{t}Z\alpha+2(Z\alpha)^{t}U\Delta U^{t}\epsilon+\epsilon^{t}U\Delta U^{t}\epsilon.
$$
Note from the law of large number for  sum of independent variables and for quadratic forms that $n^{-1}(Z\alpha)^{t}U\Delta U^{t}\epsilon\rightarrow 0$ in probability and
$$
\frac{1}{n}\left[\epsilon^{t}U\Delta U^{t}\epsilon-E\left\{\epsilon^{t}U\Delta U^{t}\epsilon\mid Z\right\}\right]\rightarrow 0  
$$
in probability. It follows that
$$
\frac{1}{n}\left[Y^{t}U\Delta U^{t}Y-(Z\alpha)^{t}U\Delta U^{t}Z\alpha-E\left\{\epsilon^{t}U\Delta U^{t}\epsilon\mid Z\right\}\right]\rightarrow 0
$$
in probability. When $\alpha=0$, $(Z\alpha)^{t}U\Delta U^{t}Z\alpha-tr(Z^{t}U\Delta U^{t}Z/p)r^{2}=0$. When $\alpha\neq 0$, it follows from the results of Bai et al (2007) that
$$
\frac{1}{n}\left\{(Z\alpha)^{t}U\Delta U^{t}Z\alpha-tr(Z^{t}U\Delta U^{t}Z/p)r^{2}\right\}\rightarrow 0, a.s.
$$
It follows from 
\begin{eqnarray*}
E\left\{\epsilon^{t}U\Delta U^{t}\epsilon\mid Z\right\}&=&(1-r^{2})\sum_{k=1}^{n}\frac{\eta_{k}-1}{(1+\lambda \eta_{k})^{2}}, \\
tr(Z^{t}U\Delta U^{t}Z/p)\sigma_{s}^{2}&=&r^{2}\sum_{k=1}^{n}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda \eta_{k})^{2}},
\end{eqnarray*}
that
\begin{eqnarray*}
\frac{1}{n}\left[Y^{t}U\Delta U^{t}Y-\sum_{k=1}^{n}\frac{\eta_{k}-1}{(1-\lambda+\lambda \eta_{k})^{2}}-r^{2}\sum_{k=1}^{n}\frac{(\eta_{k}-1)^{2}}{(1+\lambda \eta_{k})^{2}}\right]&\rightarrow&  0
\end{eqnarray*}
in probability. Hence,
$
\hat{r}_{\lambda}^{2}\rightarrow r^{2}
$ 
in probability, and thus  $\hat{\sigma}_{s}^{2}\rightarrow \sigma_{s}^{2}$ and  $\hat{\sigma}_{\epsilon}^{2}\rightarrow \sigma_{\epsilon}^{2}$ in probability. 

\vspace{0.7cm}

\noindent Proof of Theorem 2: Note that  $\sigma_{s}^{2}+\sigma_{\epsilon}^{2}=1$ and $r^{2}=\sigma_{s}^{2}$. It follows that
$$
\hat{r}_{\lambda}^{2}-r^{2}=\frac{tr\left\{W_{\lambda}(YY^{t}-M\sigma_{s}^{2}-I\sigma_{\epsilon}^{2})\right\}}
{tr\left\{W_{\lambda}(M-I)\right\}},
$$
Since 
$$
YY^{t}-M\sigma_{s}^{2}-I\sigma_{\epsilon}^{2}=Z\alpha(Z\alpha)^{t}-M\sigma_{s}^{2}+Z\alpha\epsilon^{t}+\epsilon(Z\alpha)^{t}+\epsilon\epsilon^{t}-I\sigma_{\epsilon}^{2},
$$
it follows that
\begin{eqnarray*}
\frac{1}{\sqrt{n}}tr\{W_{\lambda}(\tilde{Y}\tilde{Y}'-M\sigma_{s}^{2}-I\sigma_{\epsilon}^{2})\}&=&\frac{1}{\sqrt{n}}\left\{\alpha^{t}Z^{t}W_{\lambda}Z\alpha-\frac{1}{p}tr(Z^{t}W_{\lambda}Z)\sigma_{s}^{2}\right\}+\frac{2}{\sqrt{n}}\epsilon^{t}W_{\lambda}Z\alpha \\
&&+\frac{1}{\sqrt{n}}\left\{\epsilon^{t}W_{\lambda}\epsilon-tr(W_{\lambda})\sigma_{\epsilon}^{2}\right\},
\end{eqnarray*}
When $\alpha=0$, 
\begin{eqnarray*}
\frac{1}{\sqrt{n}}tr\{W_{\lambda}(\tilde{Y}\tilde{Y}'-M\sigma_{s}^{2}-I\sigma_{\epsilon}^{2})\}&=&\frac{1}{\sqrt{n}}\left\{\epsilon^{t}W_{\lambda}\epsilon-tr(W_{\lambda})\sigma_{\epsilon}^{2}\right\} \\
&=&\frac{1}{\sqrt{n}}\sum_{i=1}^{n}\sum_{j\neq i}W_{\lambda ij}\epsilon_{i}\epsilon_{j}+\frac{1}{\sqrt{n}}\sum_{i=1}^{n}W_{\lambda ii}(\epsilon_{i}^{2}-\sigma_{\epsilon}^{2}).
\end{eqnarray*}
Conditional on $Z$, it follows from the central limit theorems for independent variables and for the quadratic forms (de Jong, 1987 and Heyde and Brown, 1970.  See supplemental material for the condition verification) that
$$
\frac{1}{\sqrt{n}}\left(\begin{array}{c}
\sum_{i=1}^{n}\sum_{j\neq i}W_{\lambda ij}\epsilon_{i}\epsilon_{j}, \\
\sum_{i=1}^{n}W_{\lambda ii}(\epsilon_{i}^{2}-\sigma_{\epsilon}^{2})
\end{array}\right)
\rightarrow 
N\left(\left(\begin{array}{c}0\\0\end{array}\right), 
\left(\begin{array}{cc}
2\sigma_{\epsilon}^{4}(S-T) &0 \\
0 & TE(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}
\end{array}\right)\right),
$$
where
\begin{eqnarray*}
S&=&\lim _{n\rightarrow\infty}\frac{1}{n}tr(W_{\lambda}^{2})  \\ 
T&=&\lim _{n\rightarrow\infty}\frac{1}{n}\sum_{i=1}^{n}W_{\lambda ii}^{2}.
\end{eqnarray*}
It follows that
$$
\sqrt{n}(\hat{r}_{\lambda}^{2}-r^{2})\rightarrow N\left(0, \frac{2\sigma_{\epsilon}^{4}(S-T)+TE(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}}{C^{2}}\right).
$$ 

For $\alpha\neq 0$,  
$$
\frac{1}{\sqrt{n}}\left\{\alpha^{t}Z^{t}W_{\lambda}Z\alpha-\frac{1}{p}tr(Z^{t}W_{\lambda}Z)\sigma_{s}^{2}\right\}= \frac{p}{\sqrt{n}}\left\{\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}v_{k}^{2}(u)-\frac{1}{p}\sum_{k=1}^{p}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}\sigma_{s}^{2} 
$$
when $n\geq p$, and 
$$
\frac{1}{\sqrt{n}}\left\{\alpha^{t}Z^{t}W_{\lambda}Z\alpha-\frac{1}{p}tr(Z^{t}W_{\lambda}Z)\sigma_{s}^{2}\right\}= \frac{p}{\sqrt{n}}\left\{\sum_{k=1}^{n}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}v_{k}^{2}(u)-\frac{1}{p}\sum_{k=1}^{n}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}\sigma_{s}^{2}
$$
when  $n<p$.  It follows by applying Thorem 3 of Bai et al (2007) or Theorem 1.3 of Pan and Zhou (2008) that
$$
 \sqrt{\frac{p}{2}}\left\{\sum_{k=1}^{p\wedge n}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}v_{k}^{2}(u)-\frac{1}{p}\sum_{k=1}^{p\wedge n}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}\rightarrow N(0, \tau^{2}),
$$
where
$$
\tau^{2}=\int_{a}^{b} \left\{\frac{x(x-1)}{(1+\lambda x)^{2}}\right\}^{2}d\nu(x)-\left\{\int_{a}^{b} \frac{x(x-1)}{(1+\lambda x)^{2}}d\nu(x)\right\}^{2},
$$
and $\nu(x)$ is the limiting spectral measure in the Marchenko-Pastur law. It follows that
$$
\frac{1}{\sqrt{n}}\left\{\alpha^{t}Z^{t}W_{\lambda}Z\alpha-\frac{1}{p}tr(Z^{t}W_{\lambda}Z)\sigma_{s}^{2}\right\}\rightarrow N(0, 2\tau^{2}\sigma_{s}^{4}/\xi),
$$
Conditional on $Z$, it follows from the central limit theorems for independent variables and for the quadratic forms (Heyde and Brown, 1970.  See supplemental materials for the condition verification) that
$$
\frac{1}{\sqrt{n}}\left(\begin{array}{c}
\sum_{i=1}^{n}(W_{\lambda}Z\alpha)_{i}\epsilon_{i} \\
\sum_{i=1}^{n}\sum_{j\neq i}W_{\lambda ij}\epsilon_{i}\epsilon_{j} \\
\sum_{i=1}^{n}W_{\lambda ii}(\epsilon_{i}^{2}-\sigma_{\epsilon}^{2})
\end{array}\right)
\rightarrow 
N\left(\left(\begin{array}{c}0\\0\\0\end{array}\right), 
\left(\begin{array}{ccc}
 \sigma_{\epsilon}^{2}\sigma_{s}^{2}S_{1} &   0 & T_{1}E\epsilon^{3} \\
0&2\sigma_{\epsilon}^{4}(S-T) &0 \\
T_{1}E\epsilon^{3}&0 & TE(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}
\end{array}\right)\right),
$$
where 
\begin{eqnarray*}
S_{1}&=&\frac{1}{n}\lim_{n\rightarrow \infty}tr(W_{\lambda}^{t}W_{\lambda}M), \\
T_{1}&=&\lim_{n\rightarrow\infty}\frac{1}{n}\sum_{i=1}^{n}(W_{\lambda}Z\alpha)_{i}W_{\lambda ii},
\end{eqnarray*}
Together, we have
$
\sqrt{n}(\hat{r}^{2}-r^{2})\longrightarrow N(0, v_{\lambda}^{2}),
$ 
where
$$
v_{\lambda}^{2}=\frac{2\tau^{2}\sigma_{s}^{4}/\xi+4\sigma_{\epsilon}^{2}\sigma_{s}^{2}S_{1}+2\sigma_{\epsilon}^{4}S +T\{E\epsilon^{4}-3\sigma_{\epsilon}^{4}\}+2T_{1}E(\epsilon^{3})}
{C^{2}}
$$

\vspace{0.3cm}

\noindent Proof of Theorem 3: Note that $W_{*}=I-Z(Z^{t}Z)^{-1}Z^{t}$ and
\begin{eqnarray*}
\hat{r}_{*}^{2}&=&1-\frac{1}{n-p}Y^{t}\left\{I-Z(Z^{t}Z)^{-1}Z^{t}\right\}Y. \\
&=&1-\frac{1}{n-p}\epsilon^{t}\left\{I-Z(Z^{t}Z)^{-1}Z^{t}\right\}\epsilon. 
\end{eqnarray*}
 Since for fixed symmetric matrix $A=(a_{ij})_{n\times n}$,
$$
E(\epsilon A\epsilon)^{2}=\sum_{i=1}^{n}a_{ii}^{2}(E\epsilon^{4}-3\sigma_{\epsilon}^{4})+\left[2tr(A^{2})+\{tr(A)\}^{2}\right]\sigma_{\epsilon}^{4}.
$$
It follows that, 
\begin{eqnarray*}
E\left\{|\hat{r}_{*}^{2}-r^{2}|^{2}\mid Z\right\}&=&\frac{1}{(n-p)^{2}}\sum_{i=1}^{n}a_{ii}^{2}\left(E\epsilon^{4}-3\sigma_{\epsilon}^{4}\right)+\frac{2}{n-p}\sigma_{\epsilon}^{4} \\
&\leq&\frac{1}{n-p}\left(E\epsilon^{4}-\sigma_{\epsilon}^{4}\right)\rightarrow 0,
\end{eqnarray*}
because $n-p=n(1-1/\xi)\rightarrow \infty$. It follows that $\hat{r}_{*}^{2}\rightarrow r^{2}$ in probability.

Conditional on $Z$, it follows from the central limit theorems for independent variables and for the quadratic forms (de Jong, 1987 and Heyde and Brown, 1970) that
$$
\frac{1}{\sqrt{n}}\left(\begin{array}{c}
\sum_{i=1}^{n}\sum_{j\neq i}W_{* ij}\epsilon_{i}\epsilon_{j}, \\
\sum_{i=1}^{n}W_{* ii}(\epsilon_{i}^{2}-\sigma_{\epsilon}^{2})
\end{array}\right)
\rightarrow 
N\left(\left(\begin{array}{c}0\\0\end{array}\right), 
\left(\begin{array}{cc}
2\sigma_{\epsilon}^{4}(S_{*}-T_{*}) &0 \\
0 & T_{*}E(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}
\end{array}\right)\right),
$$
where
\begin{eqnarray*}
S_{*}&=&\lim _{n\rightarrow\infty}\frac{1}{n}tr(W_{*}^{2}) =1-1/\xi, \\ 
T_{*}&=&\lim _{n\rightarrow\infty}\frac{1}{n}\sum_{i=1}^{n}W_{* ii}^{2}=.
\end{eqnarray*}
It follows that
$$
\sqrt{n}(\hat{r}_{*}^{2}-r^{2})\rightarrow N\left(0, \frac{2\sigma_{\epsilon}^{4}S_{*}+T_{*}(E\epsilon^{4}-3\sigma_{\epsilon}^{4})}{(1-1/\xi)^{2}}\right).
$$ 


\begin{center} Appendix II: Variance estimates\end{center}

\vspace{0.3cm}

When $\alpha=0$, the numerator in the $v^{2}$ expression can be approximated by
$$
\frac{2\sigma_{\epsilon}^{4}}{n}tr(W^{t}W)+\frac{1}{n}\sum_{i=1}^{n}W_{ii}^{2}\left\{E(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}-2\sigma_{\epsilon}^{4}\right\},
$$
which can be consistently estimated by
$$
\frac{2}{n}\left\{tr(W^{t}W)-\sum_{i=1}^{n}W_{ii}^{2}\right\}+\frac{1}{n}\sum_{i=1}^{n}W_{ii}^{2}(Y_{i}^{2}-1)^{2}.
$$

In general, to estimate the variance $v^{2}$, note that $C$ can be consistently estimated by $tr\{W(M-I)\}/n$. The first term in the numerator can be consistently estimated by $2\hat{r}^{4}\hat{\tau}^{2}p/n$, where
$$
\hat{\tau}^{2}=\frac{1}{p}\sum_{k=1}^{p\wedge n}\left\{\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}^{2}-\left\{\frac{1}{p}\sum_{k=1}^{p\wedge n}\frac{\eta_{k}(\eta_{k}-1)}{(1+\lambda\eta_{k})^{2}}\right\}^{2}.
$$
The second term in the numerator can be consistently estimated by $4\hat{r}^{2}(1-\hat{r}^{2})tr(W^{t}WM)/n$. The first part of the third term ($2\sigma_{\epsilon}^{2}S$) in the numerator can be consistently estimated by $2(1-\hat{r}^{2})^{2}tr(W^{t}W)/n$. 
When $\epsilon$ follows the normal distribution, the rest terms in the numerator, i.e., 
$$
T\{E(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}-2\sigma_{\epsilon}^{4})+2T_{1}E(\epsilon^{3})=0.
$$
As a result,
$$
\tilde{v}^{2}=\frac{2\hat{r}^{4}\hat{\tau}^{2}p/n+4\hat{r}^{2}(1-\hat{r}^{2})tr(W^{t}WM)/n+2(1-\hat{r}^{2})^{2}tr(W^{t}W)/n}{[tr\{W(M-I)\}/n]^{2}},
$$
is a consistent estimate of the variance under the normal random error. 
  
For non-zero $\alpha$ and possibly non-normal random error in general, note that
$$
Y_{i}^{2}-1-(M_{ii}-1)\sigma_{s}^{2}=\epsilon_{i}^{2}-\sigma_{\epsilon}^{2}+2\epsilon_{i}z_{i}^{t}\alpha+(z_{i}^{t}\alpha)^{2}-M_{ii} \sigma_{s}^{2}.
$$
It follows that
\begin{eqnarray*}
\sum_{i=1}^{n}E\{Y_{i}^{2}-1-(M_{ii}-1)\sigma_{s}^{2}\}^{2}&=&\sum_{i=1}^{n}E\{\epsilon_{i}^{2}-\sigma_{\epsilon}^{2}\}^{2}+4n\sigma_{s}^{2}\sigma_{\epsilon}^{2}
+\sum_{i=1}^{n}E\{(z_{i}^{t}\alpha)^{2}-M_{ii} \sigma_{s}^{2}\}^{2}.
\end{eqnarray*}
Note that 
$$
\sum_{i=1}^{n}E\{(z_{i}^{t}\alpha)^{2}-M_{ii} \sigma_{s}^{2}\}^{2}=\sum_{i=1}^{n}E\left\{M_{ii}-(z_{i}^{t}u)^{2}\right\}^{2}\sigma_{s}^{4},
$$
where $||u||_{2}=1$. An estimated upper bound for $E(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}$ is
$$
\frac{1}{n}\sum_{i=1}^{n}\{Y_{i}^{2}-1-(M_{ii}-1)\hat{r}^{2}\}^{2} -4\hat{r}^{2}(1-\hat{r}^{2})-g\hat{r}^{4},
$$ 
where
$$
g=\min _{||u||_{2}=1}\frac{1}{n}\sum_{i=1}^{n}E\{(z_{i}^{t}u)^{2}-M_{ii}\}^{2}.
$$
For simplicity of calculation, we may take $g=0$. Recall that $M_{ii}=p^{-1}\sum_{j=1}^{p}Z_{ij}^{2}$. Direct calculation shows that
$$
\sum_{i=1}^{n}E\left\{M_{ii}-(z_{i}^{t}u)^{2}\right\}^{2}=\sum_{i=1}^{n}\left\{2+\sum_{j=1}^{p}u_{j}^{4}(EZ_{ij}^{4}-3)+p^{-1}\sum_{j=1}^{p}(p^{-1}-2u_{j}^{2})E(Z_{ij}^{4}-1)\right\}.
$$
The last term on the right-hand side is negligible relative to other terms when $p$ is large. For $EZ_{ij}^{4}=3$ the second term is $0$. When $EZ_{ij}^{4}=3$, a consistent estimate of $E(\epsilon^{2}-\sigma_{\epsilon}^{2})^{2}$ can be obtained as
$$
\frac{1}{n}\sum_{i=1}^{n}\{Y_{i}^{2}-1-(M_{ii}-1)\hat{r}^{2}\}^{2} -4\hat{r}^{2}(1-\hat{r}^{2})-2\hat{r}^{4}
$$ 
This suggests that when $E\epsilon^{3}=0$, a consistent estimate of the asymptotic variance for $\sqrt{n}(\hat{r}^{2}-r^{2})$ is
$\hat{v}^{2}=\tilde{v}^{2}+\widehat{va}$, where
$$
\widehat{va}=\frac{\frac{1}{n}\sum_{i=1}^{n}\{Y_{i}^{2}-1-(M_{ii}-1)\hat{r}^{2}\}^{2} -4\hat{r}^{2}(1-\hat{r}^{2})-2\hat{r}^{4}}{[tr\{W(M-I)\}/n]^{2}}\frac{1}{n}\sum_{i=1}^{n}W_{ii}^{2}.
$$
Because $\widehat{va}$ is not guaranteed to be postive while the estimand is positive, we proposed to use $\hat{v}^{2}=\tilde{v}^{2}+\widehat{va}1_{\{\widehat{va}\geq 0\}}$ instead. 


\begin{comment}
 An alternative approach uses simulation. Let $\delta_{t1},\cdots,\delta_{tn}$ be independent normal random variables with mean $0$ and variance $\sigma_{t}^{2}$. Let 
$$
Y_{ti}=Y_{i}+\delta_{ti}.
$$
The proportion of variance $Y_{t}$ explained by the covariate $Z$ is
$$
r_{t}^{2}=\frac{\sigma_{s}^{2}}{\sigma_{s}^{2}+\sigma_{\epsilon}^{2}+\sigma_{t}^{2}}=\frac{r^{2}}{1+\sigma_{t}^{2}/\mbox{var}(Y)}.
$$
It can be shown that the estimator of $r_{t}^{2}$, $\hat{r}^{2}$ asymptotically follows a normal distribution as
$$
\sqrt{n}(\hat{r}_{t}^{2}-r_{t}^{2})\longrightarrow N(0,v_{t}^{2}),
$$
where
\begin{eqnarray*}
v_{t}^{2}&=&\frac{2\tau^{2}\sigma_{s}^{4}/\xi+4(\sigma_{\epsilon}^{2}+\sigma_{t}^{2})\sigma_{s}^{2}S_{1}+2(\sigma_{\epsilon}^{2}+\sigma_{t}^{2})^{2}S +T\{E(\epsilon+\delta_{t})^{4}-3(\sigma_{\epsilon}^{2}+\sigma_{t}^{2})^{2}\}+2T_{1}E(\epsilon+\delta_{t})^{3}}{C^{2}}  \\
&=&v^{2}+\frac{4\sigma_{t}^{2}\sigma_{s}^{2}S_{1}+2(2\sigma_{\epsilon}^{2}\sigma_{t}^{2}+\sigma_{t}^{4})S -2T\sigma_{\epsilon}^{2}\sigma_{t}^{2}}{C^{2}}. 
\end{eqnarray*}
It can be seen that
$$
\widehat{ev}_{t}^{2}=\left\{\sqrt{n}(\hat{r}_{t}^{2}-r_{t}^{2})\right\}^{2}-\frac{4\sigma_{t}^{2}\sigma_{s}^{2}S_{1}+2(2\sigma_{\epsilon}^{2}\sigma_{t}^{2}+\sigma_{t}^{4})S -2T\sigma_{\epsilon}^{2}\sigma_{t}^{2}}{C^{2}}
$$ 
is an approximately unbiased estimating score for $v^{2}$. Tne simulation approach can be carried out as follows. For $t=1,\cdots,m$, choose a set of $\sigma_{t}^{2}$ in increasing order. Performing the simulation to obtain $\widehat{ev}_{t}, t=1,\cdots,m$. Estimate $v^{2}$ by
$$
\widehat{ev}^{2}=\frac{1}{m}\sum_{t=1}^{m}\widehat{ev}_{t}^{2}.
$$
{\bf This may not work as true $r^{2}$ is not known and plugging-in the estimated can change the variance expression.} 
\end{comment}














